The Erlang Weighted Tree, A New Branching Process

In this paper, we study a new discrete tree and the resulting branching process, which we call the \textbf{E}rlang \textbf{W}eighted \textbf{T}ree(\textbf{EWT}). The EWT appears as the local weak limit of a random graph model proposed in~\cite{La2015}. In contrast to the local weak limit of well-known random graph models, the EWT has an interdependent structure. In particular, its vertices encode a multi-type branching process with uncountably many types. We derive the main properties of the EWT, such as the probability of extinction, growth rate, etc. We show that the probability of extinction is the smallest fixed point of an operator. We then take a point process perspective and analyze the growth rate operator. We derive the Krein--Rutman eigenvalue $\beta_0$ and the corresponding eigenfunctions of the growth operator, and show that the probability of extinction equals one if and only if $\beta_0 \leq 1$.

==> Sections/PropEWT/Extincbeta.tex <==
The value of $\beta_0$ obtained in section \ref{sec:PFeigenvalue}, provides an easy way to check whether the probability of extinction equals 1 or not. The first step to derive the relation between the probability of extinction and $\beta_0$ is to show that $Z_l$, the number of nodes at generation $l$, cannot stay bounded and non-zero infinitely often.
\begin{theorem}\label{thm:boundedZ}
	For any finite value $M>0$, and any choice of $(x,m)\in \mathbb{R}\times \mathbb{N}$,
	\begin{align*}
	\prob\left( 0< Z_l \leq M \text{ infinitely often}| n_\phi = m, v_\phi = x\right) = 0
	\end{align*}
	where $Z_l$ denote the number of nodes at generation $l$.
\end{theorem}
In order to prove the Theorem \ref{thm:boundedZ}, we need to show that given a node of type $(x,m)$, the probability that its descendants will extinct after two generations is uniformly positive for any fixed value of $m$. Note that given the type of a node in EWT, survival of its descendants is independent of the rest of the tree. Moreover, the corresponding probability is the same as if the node was the root node.
\begin{lemma}
	Consider a node of type $(x,m)$, the probability that its decedents extinct after at most two generations is bounded below by $\epsilon ^m$ for some $\epsilon > 0$ independent of $m$ and $x$.
\end{lemma}
\begin{proof}[proof of lemma]
	Based on the proof of the Theorem \ref{thm:probext},
	\begin{align*}
	\prob(Z_{2} = 0 | n_\phi = m, v_{\phi} = x) = \left(T^2(\boldsymbol{0})(x)\right)^m
	\end{align*}
	Moreover, the function $T^2(\boldsymbol{f})(\cdot)$ is non-decreasing(part i of Lemma \ref{lem:propt}); hence, the right hand side of the above equality obtains its minimum at $x = 0$ and we have,
	\begin{align*}
	\prob(Z_{2} = 0 | n_\phi = m, v_{\phi} = x) \geq \left(T^2(\boldsymbol{0})(0)\right)^m = \left(\sum_{k=1}^{\infty}P(k) \int_{0}^{\infty}\frac{e^{-z}z^{k-1}}{(k-1)!}\left(T(\boldsymbol{0})(z)\right)^{k-1}dz\right)^m
	\end{align*}
	Finally, set $\epsilon>0$ to be the term in the parenthesis of the right-hand side.
\end{proof}
\begin{proof}[proof of theorem]
	content...
\end{proof}
